Translating Canonical SQL to Imperative Code in Coq

SQL is by far the most widely used and implemented query language. Yet, on some key features, such as correlated queries and NULL value semantics, many implementations diverge or contain bugs. We leverage recent advances in the formalization of SQL and query compilers to develop DBCert, the first mechanically verified compiler from SQL queries written in a canonical form to imperative code. Building DBCert required several new contributions which are described in this paper. First, we specify and mechanize a complete translation from SQL to the Nested Relational Algebra which can be used for query optimization. Second, we define Imp, a small imperative language sufficient to express SQL and which can target several execution languages including JavaScript. Finally, we develop a mechanized translation from the nested relational algebra to Imp, using the nested relational calculus as an intermediate step.

==> fig/correlated-ex.tex <==
  \begin{minipage}[c]{.6\linewidth}
    \centering
    \smaller
    Database example\hspace{1cm}\Sql{T1}~
    \begin{tabular}{|c|c|}
      \hline
      a1 & b1 \\
      \hline
      1 & 1\\
      1 & 2\\
      2 & 3\\
      3 & 1\\
      3 & 2 \\
        3 & 3\\
      \hline
    \end{tabular}
    \hspace{1cm}\Sql{T2}~
    \begin{tabular}{|c|c|}
      \hline
      a2 & b2 \\
          \hline
      7 & 7\\
      7 & 8 \\
      \hline          
    \end{tabular}
  \end{minipage} 
  \begin{minipage}[c]{.20\linewidth}
    \centering
    \smaller
    \hfill
  \end{minipage}
  
  \begin{minipage}[c]{.9\linewidth}
    \Sql{Q1}\hspace{.2cm}
  \begin{minipage}[c]{.45\linewidth}
    \begin{lstlisting}[language=SQLL]
select a1 from t1 group by a1 having exists
  (select a2 from t2 group by a2 having
   sum(1+0*a2) = 2);
\end{lstlisting}
  \end{minipage}
  \begin{minipage}[l]{.45\linewidth}
    \centering\smaller
    The corresponding result~\hspace{.2cm}
    \begin{tabular}{|c|}
      \hline
      a1  \\
      \hline
      1 \\ 2 \\3 \\
      \hline          
    \end{tabular}  
  \end{minipage}
  \end{minipage}
  
  \begin{minipage}[c]{.9\linewidth}
    \Sql{Q2}\hspace{.2cm}
  \begin{minipage}[c]{.45\linewidth}
    \begin{lstlisting}[language=SQLL]
select a1 from t1 group by a1 having exists
  (select a2 from t2 group by a2 having
   sum(1+0*a1) = 2);
\end{lstlisting}
  \end{minipage}
  \begin{minipage}[c]{.45\linewidth}    
    \centering\smaller    
    The corresponding result~\hspace{.2cm}
    \begin{tabular}{|c|}
      \hline
      a1  \\
      \hline
      1 \\
      \hline          
    \end{tabular}  
  \end{minipage}
  \end{minipage}

%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:


==> fig/correlated-translation-ex.tex <==
  \begin{minipage}[c]{.9\linewidth}
    \Sql{Q1}\hspace{.2cm}
  \begin{minipage}[c]{.45\linewidth}
    \begin{lstlisting}[language=SQLL]
select a1 from t1 group by a1 having exists
 (select a2 from t2 group by a2 having
   sum(1+0*a2) = 2);
\end{lstlisting}
  \end{minipage}
  \begin{minipage}[l]{.45\linewidth}
    \centering
    {\smaller
     GlobOp1 ({\tt sum} (GlobOp2 {\tt a2}))}
  \end{minipage}
  \end{minipage}
  
  \begin{minipage}[c]{.9\linewidth}
    \Sql{Q2}\hspace{.2cm}
  \begin{minipage}[c]{.45\linewidth}
    \begin{lstlisting}[language=SQLL]
select a1 from t1 group by a1 having exists
  (select a2 from t2 group by a2 having
   sum(1+0*a1) = 2);
\end{lstlisting}
  \end{minipage}
  \begin{minipage}[c]{.45\linewidth}    
    \centering
    {\smaller
    GlobOp1 ({\tt sum} (GlobOp2~{\tt a1}) \eapp{}{}\qENV.$\mathit{tail}$)}
  \end{minipage}
\end{minipage}


%%% Local Variables: 
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End: 


==> fig/imp-semantics.tex <==

  \centering
  \smaller
  $$
  \begin{array}[t]{lcl}
    \impsem{c}{\envimp} & = & c
    \\[0.2em]
    \impsem{x}{\envimp} & = & \envimp(x)
    \\[0.2em]
    \impsem{\mathit{op}(e)}{\envimp} & = & \impdatasem{\mathit{op}(\impsem{e}{\envimp})}
    \\[0.2em]
    \impsem{\mathit{f}(e)}{\envimp} & = & \impdatasem{\mathit{f}(\impsem{e}{\envimp})}
    \\[0.5em]

    \impsem{\impassign{x}{e}}{\envimp} & = &
       \envimp[x \leftarrow \impsem{e}{\envimp}]
    \\[0.2em]

    \impsem{\impif{e}{s_1}{s_2}}{\envimp} & = &
       % \\ \multicolumn{3}{l}{ \qquad
         \algoif{\tobool{\impsem{e}{\envimp}}}{\impsem{s_1}{\envimp}}{\impsem{s_2}{\envimp}}
       % }
    \\[0.2em]

    \impsem{\impforrange{x}{e}{s}}{\envimp} & = &
       % \\ \multicolumn{3}{l}{ \qquad
         \algofold{(\lambda(\envimp, c). \impsem{s}{\envimp[x \leftarrow c]})}{\envimp}{(\tolist{\impsem{e}{\envimp}})}
       % }
    \\[0.2em]

    \impsem{\impblock{\mathit{decls}\ \mathit{stmts}}}{\envimp} & = &
       \impsem{\mathit{stmts}}{\impsem{\mathit{decls}}{\envimp}}
         \backslash \mathit{Dom}(\mathit{decls})
    \\[0.2em]
    \impsem{s\ \mathit{stmts}}{\envimp} & = & \impsem{\mathit{stmts}}{\impsem{s}{\envimp}}
    \\[0.2em]
    \impsem{\epsilon}{\envimp} & = & \envimp
  \end{array}
  $$

  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> fig/instantiation-elements.tex <==
  \small
  \[
    \begin{array}[c]{|c|c|}
      \hline
      \text{\bf Abstract in \sqlalg}
      & \text{\bf Assumed in the specification of the translation} \\
      \hline
      \begin{array}{c}
        \smaller
        {\attribute}: \text{Domain of attribute names} \\
        <_a: \text{Order on attributes}
        \end{array} 
      & 
        \begin{array}{c}
          \tratt{\_}: \text{Translation function}\\
          \forall l_1 l_2, l_1  <_a l_2 \rightarrow
          \tratt{l_1} <_d \tratt{l_2}\\
        \end{array} \\
      \hline
      \begin{array}{c}
        \smaller
          \val: \text{Domain of values} \\
        \end{array} 
      & 
        \begin{array}{c}
          \trval{\_}: 
          \text{Translation function} \\
          \forall v_1 v_2, \trval{v_1} = \trval{v_2} \rightarrow
          v_1 = v_2\\
        \end{array} \\
      \hline
      \begin{array}{c}
        \smaller
        \predicate: \text{Abstract predicate symbols} \\
        \end{array} 
      & 
        \begin{array}{c}
          \trp{p}{\_}: \text{Translation function}\\
          \forall p,
          ( \vdash \trp{p}{\overline{\Tau_{x}(x)}} \Downarrowa
          \trval{\interp{p}_{b} (\overline{\interp{x}})}) \\
        \end{array} \\
      \begin{array}{c}
        \smaller
        \function: \text{Abstract function symbols} \\
        \end{array} 
      & 
        \begin{array}{c}
          \trfn{\fn}{\_}: \text{Translation function} \\
          \forall \fn,
          ( \vdash \trfn{\fn}{\overline{\Tau_{x}(x)}} \Downarrowa
          \trval{\interp{\fn}_{f} (\overline{\interp{x}})})\\
        \end{array} \\
      
      \hline
      \begin{array}{c}
        \smaller
        \aggregate: \text{Abstract aggregate symbols} \\
        \end{array} 
      & 
        \begin{array}{c}
          \trag{\ag}{\_}: \text{Translation function}\\
          \forall \ag,
          ( \vdash \trag{\ag}{\overline{\Tau_{x}(x)}} \Downarrowa
          \trval{\interp{\ag}_{a} (\overline{\interp{x}})}) \\
        \end{array} \\
      \hline
      \text{Three-valued logic}
      &
        \begin{array}{c}
          \neg_B,\wedge_B,\vee_B$, ${\tt is\_true}_B, \text{\tt in}:
          \text{Abstract operators} \\
          \text{The corresponding semantics preservation lemmas}\\
        \end{array} \\
      \hline
    \end{array}
  \]
%%% Local Variables: 
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End: 


==> fig/nrae-semantics-denot.tex <==

\newcommand{\semnra}[3]{\ensuremath{\llbracket#1\rrbracket^{\mbox{\tiny
        \nrae}}_{<#2,#3>}}}
\newcommand{\semuop}[1]{\ensuremath{\llbracket#1\rrbracket^{\mbox{\tiny uop}}}}
\newcommand{\sembop}[1]{\ensuremath{\llbracket#1\rrbracket^{\mbox{\tiny bop}}}}
\newcommand{\qid}{\texttt{In}}
\newcommand{\qenv}{\texttt{Env}}

\[
  \begin{array}{llll}
  \semnra{c}{\envnraenv}{d} &=& c&\\
  \semnra{\qid}{\envnraenv}{d} &=& d&\\
  \semnra{\qenv}{\envnraenv}{d} &=& \envnraenv&\\
  \semnra{q_2 \circ^e q_1}{\envnraenv}{d} &=&
  \semnra{q_2}{\semnra{q_1}{\envnraenv}{d}}{d}&\\
  \semnra{\opunop\, q}{\envnraenv}{d} &=& \semuop{\opunop}
  \semnra{q}{\envnraenv}{d}&\\
    \semnra{q_1 \opbinop q_2}{\envnraenv}{d} &=& \semnra{q_1}{\envnraenv}{d}
    \sembop{\opbinop} \semnra{q_2}{\envnraenv}{d}&\\
    \semnra{q_2 \circ q_1}{\envnraenv}{d}
                        &=& 
                            \semnra{q_2}{\envnraenv}{\semnra{q_1}{\envnraenv}{d}}
                             &\\
    
                        &&   &  \\       
                             %% cartesian
    \semnra{\emptyset \times q_2}{\envnraenv}{d}
                        &=&
                            \emptyset& \\
    \semnra{q_1 \times \emptyset}{\envnraenv}{d}
                        &=&
                            \emptyset& \\
    \semnra{q_1 \times q_2}{\envnraenv}{d}
                        &=&
                            \{d_1 \opconcat d_2\}\cup& \mbox{if}~\semnra{
                           q_1}{\envnraenv}{d} =
                           \{d_1\}\!\cup\! s_1\\
                        &&
                            \semnra{
                           \{d_1\}\!\times\! s_2}{\envnraenv}{d}\cup & \mbox{and}~
                           \semnra{
                           q_2}{\envnraenv}{d} =
                           \{d_2\}\!\cup\! s_2\\
                        &&
                            \semnra{s_1\!\times\! \left(\{d_2\}\!\cup\! 
                            s_2\right) }{\envnraenv}{d}          
                             & \\
                        &&   &  \\       
                       % map
    \semnra{\qmap{q_2}{q_1}}{\envnraenv}{d}
                        &=&
                            \emptyset
                              &
                               \mbox{if}~\semnra{q_1}{\envnraenv}{d} = \emptyset\\
      \semnra{\qmap{q_2}{q_1}}{\envnraenv}{d}
                        &=&
                            [\semnra{q_2}{\envnraenv}{d_1}] \cup
                            \semnra{\qmap{q_2}{s_1}}{\envnraenv}{d} &
                               \mbox{if}~\semnra{q_1}{\envnraenv}{d} =
                               [d_1] \cup s_1\\
                        && &\\  %% select
      \semnra{\qselect{q_2}{q_1}}{\envnraenv}{d}
      &=&
          \emptyset & \mbox{if}~\semnra{q_1}{\envnraenv}{d} =
          \emptyset\\ 
      \semnra{\qselect{q_2}{q_1}}{\envnraenv}{d}
      &=&
          \semnra{\qselect{q_2}{s_1}}{\envnraenv}{d} 
                             &
                               \begin{array}{l}
                                 \mbox{if}~\semnra{q_1}{\envnraenv}{d} =
                                 [d_1] \cup s_1\\ 
                                 \mbox{and}~\semnra{q_2}{\envnraenv}{d_1}
                                 = \texttt{false}  
                               \end{array}\\
              
     
          \semnra{\qselect{q_2}{q_1}}{\envnraenv}{d}
      &=&
          [d_1] \cup
          \semnra{\qselect{q_2}{s_1}}{\envnraenv}{d} &
                                                   \begin{array}{l}
                                                     \mbox{if}~\semnra{q_1}{\envnraenv}{d}
                                                     = [d_1] \cup
                                                     s_1\\
                                                     
                                                     \mbox{and}~\semnra{q_2}{\envnraenv}{d_1}
                                                     = \texttt{true}
                                                     
                                                     \end{array}\\
              
      && & \\ 
      %either
      \semnra{\qeither{q_1}{q_2}}{\envnraenv}{\dleft{}~d}
      &=&
          \semnra{q_1}{\envnraenv}{d}\\
      \semnra{\qeither{q_1}{q_2}}{\envnraenv}{\dright{}~d}
      &=&
          \semnra{q_2}{\envnraenv}{d}
    \end{array}
\]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> fig/nrae-semantics-summary.tex <==
  \begin{minipage}[l]{\textwidth}
{\footnotesize
  \begin{gather*}
    \infer[Constant]
    {\envnraenv \vdash d_0 \qapp\ d \Downarrowa d_0}
    {}
    \qquad
    \infer[ID]
    {\envnraenv \vdash \qID \qapp\ d \Downarrowa d}
    {}
    \qquad
    \infer[Comp]
    {\envnraenv \vdash q_2 \circ q_1 \qapp\ d_0 \Downarrowa d_2}
    {\envnraenv \vdash q_1 \qapp\ d_0 \Downarrowa d_1
     \quad
     \envnraenv \vdash q_2 \qapp\ d_1 \Downarrowa d_2}
    \\[\jot]
    % \infer[Unary]
    % {\envnraenv \vdash \opunop\, q \qapp d \Downarrowa d_1}
    % {\envnraenv \vdash q \qapp d \Downarrowa d_0
    %  \quad
    %  \opunop\, d_0 = d_1}
    % \qquad
    % \infer[Binary]
    % {\envnraenv \vdash q_1\opbinop q_2 \qapp d \Downarrowa d_3}
    % {\envnraenv \vdash q_1 \qapp d \Downarrowa d_1
    %  \quad
    %  \envnraenv \vdash q_2 \qapp d \Downarrowa d_2
    %  \quad
    %  \envnraenv \vdash d_1\opbinop d_2 = d_3}
    % \\[\jot]
    % \infer[Map~\emptyset]
    % {\envnraenv \vdash \qmap{q_2}{q_1} \qapp d \Downarrowa \emptyset}
    % {\envnraenv \vdash q_1 \qapp d \Downarrowa \emptyset}
    % \qquad
    % \infer[Map]
    % {\envnraenv \vdash \qmap{q_2}{q_1} \qapp d \Downarrowa [d_2]\cup s_2}
    % {\envnraenv \vdash q_1 \qapp d \Downarrowa [d_1]\cup s_1
    %  \quad
    %  \envnraenv \vdash q_2 \qapp d_1 \Downarrowa d_2
    %  \quad
    %  \envnraenv \vdash \qmap{q_2}{s_1} \qapp d \Downarrowa s_2}
    % \\[\jot]
    % \infer[Sel_{\mbox{T}}]
    % {\envnraenv \vdash \qselect{q_2}{q_1} \qapp d \Downarrowa [d_1]\cup s_2}
    % {\envnraenv \vdash q_1 \qapp d \Downarrowa [d_1]\cup s_1
    %  \quad
    %  \envnraenv \vdash q_2 \qapp d_1 \Downarrowa \true
    %  \quad
    %  \envnraenv \vdash \qselect{q_2}{s_1} \qapp d \Downarrowa s_2}
    % \\[\jot]
    % \infer[Sel_{\mbox{F}}]
    %   {\envnraenv \vdash \qselect{q_2}{q_1} \qapp d \Downarrowa s_2}
    %   {\envnraenv \vdash q_1 \qapp d \Downarrowa [d_1]\cup s_1
    %    \quad
    %    \envnraenv \vdash q_2 \qapp d_1 \Downarrowa \false
    %    \quad
    %    \envnraenv \vdash \qselect{q_2}{s_1} \qapp d \Downarrowa s_2}
    % \qquad
    % \infer[Sel_\emptyset]
    %   {\envnraenv \vdash q_1 \qapp d \Downarrowa \emptyset}
    %   {\envnraenv \vdash \qselect{q_2}{q_1} \qapp d \Downarrowa \emptyset}
    % \\[\jot]
    % \infer[Prod^{l}_{\emptyset}]
    %   {\envnraenv \vdash q_1\times q_2 \qapp d \Downarrowa \emptyset}
    %   {\envnraenv \vdash q_1 \qapp d \Downarrowa \emptyset}
    % \qquad
    % \infer[Prod^{r}_{\emptyset}]
    %   {\envnraenv \vdash q_1\times q_2 \qapp d \Downarrowa \emptyset}
    %   {\envnraenv \vdash q_2 \qapp d\Downarrowa \emptyset}
    % \\[\jot]
    % \infer[Prod]
    %   {\envnraenv \vdash q_1\times q_2 \qapp d \Downarrowa [d_1 \opconcat d_2]\cup s_3\cup s_4}
    %   {\envnraenv \vdash q_1 \!\qapp\! d\!\Downarrowa\! [d_1]\!\cup\! s_1
    %    \quad
    %    \envnraenv \vdash q_2 \!\qapp\! d\!\Downarrowa\! [d_2]\!\cup\! s_2
    %    \quad
    %    \envnraenv \vdash [d_1]\!\times\! s_2 \!\qapp\! d\!\Downarrowa\! s_3
    %    \quad
    %    \envnraenv \vdash s_1\!\times\! \left([d_2]\!\cup\! s_2\right) \!\qapp\! d\! \Downarrowa\! s_4}
    % \\[\jot]
    \infer[Env]
      {\envnraenv \vdash \qENV \qapp\ d \Downarrowa \envnraenv}
      {}
    \qquad
    \infer[\mbox{Comp$^e$}]
      {\envnraenv_1 \vdash q_2 \circ^e q_1 \qapp\ d_1 \Downarrowa d_2}
      {\envnraenv_1 \vdash q_1 \qapp\ d_1 \Downarrowa \envnraenv_2
       \quad
       \envnraenv_2 \vdash q_2 \qapp\ d_1 \Downarrowa d_2}
    \\[\jot]
    % \infer[\mbox{Map$^e_\emptyset$}]
    %   {\emptyset \vdash \qmapenv{q_2} \qapp d \Downarrowa \emptyset}
    %   {}
    % \qquad
    % \infer[\mbox{Map$^e$}]
    %   {[d_1]\cup s_1 \vdash \qmapenv{q_2} \qapp d \Downarrowa [d_2]\cup s_2}
    %   {d_1 \vdash q_2 \qapp d \Downarrowa d_2
    %    \quad
    %    s_1 \vdash \qmapenv{q_2} \qapp d \Downarrowa s_2}
    % \\[\jot]
    % \infer[\mbox{Default$_{\lnot\emptyset}$}]
    %   {\envnraenv \vdash q_1~\qor~q_2\qapp d \Downarrowa d_1}
    %   {\envnraenv \vdash q_1\qapp d \Downarrowa d_1
    %    \quad
    %    d_1 \neq \emptyset}
    % \qquad
    % \infer[\mbox{Default$_{\emptyset}$}]
    %   {\envnraenv \vdash q_1~\qor~q_2\qapp d \Downarrowa d_2}
    %   {\envnraenv \vdash q_1\qapp d \Downarrowa \emptyset
    %    \quad
    %    \envnraenv \vdash q_2\qapp d \Downarrowa d_2}
    % \\[\jot]
    \infer[\mbox{Either$_{\dleft{}}$}]
      {\envnraenv \vdash \qeither{q_1}{q_2}\qapp {\dleft{}}\ d \Downarrowa d_1}
      {\envnraenv \vdash q_1\qapp d \Downarrowa d_1}
    \qquad
    \infer[\mbox{Either$_{\dright{}}$}]
      {\envnraenv \vdash \qeither{q_1}{q_2}\qapp {\dright{}}\ d \Downarrowa d_2}
      {\envnraenv \vdash q_2\qapp d \Downarrowa d_2}
  \end{gather*}
}
\end{minipage}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> fig/nrae-semantics.tex <==
  \begin{minipage}[l]{\textwidth}
{\footnotesize
  \begin{gather*}
    \infer[Constant]
    {\envnraenv \vdash d_0 \qapp\ d \Downarrowa d_0}
    {}
    \qquad
    \infer[ID]
    {\envnraenv \vdash \qID \qapp\ d \Downarrowa d}
    {}
    \qquad
    \infer[Comp]
    {\envnraenv \vdash q_2 \circ q_1 \qapp\ d_0 \Downarrowa d_2}
    {\envnraenv \vdash q_1 \qapp\ d_0 \Downarrowa d_1
     \quad
     \envnraenv \vdash q_2 \qapp\ d_1 \Downarrowa d_2}
    \\[\jot]
    \infer[Unary]
    {\envnraenv \vdash \opunop\, q \qapp d \Downarrowa d_1}
    {\envnraenv \vdash q \qapp d \Downarrowa d_0
     \quad
     \opunop\, d_0 = d_1}
    \qquad
    \infer[Binary]
    {\envnraenv \vdash q_1\opbinop q_2 \qapp d \Downarrowa d_3}
    {\envnraenv \vdash q_1 \qapp d \Downarrowa d_1
     \quad
     \envnraenv \vdash q_2 \qapp d \Downarrowa d_2
     \quad
     \envnraenv \vdash d_1\opbinop d_2 = d_3}
    \\[\jot]
    \infer[Map~\emptyset]
    {\envnraenv \vdash \qmap{q_2}{q_1} \qapp d \Downarrowa \emptyset}
    {\envnraenv \vdash q_1 \qapp d \Downarrowa \emptyset}
    \qquad
    \infer[Map]
    {\envnraenv \vdash \qmap{q_2}{q_1} \qapp d \Downarrowa [d_2]\cup s_2}
    {\envnraenv \vdash q_1 \qapp d \Downarrowa [d_1]\cup s_1
     \quad
     \envnraenv \vdash q_2 \qapp d_1 \Downarrowa d_2
     \quad
     \envnraenv \vdash \qmap{q_2}{s_1} \qapp d \Downarrowa s_2}
    \\[\jot]
    \infer[Sel_{\mbox{T}}]
    {\envnraenv \vdash \qselect{q_2}{q_1} \qapp d \Downarrowa [d_1]\cup s_2}
    {\envnraenv \vdash q_1 \qapp d \Downarrowa [d_1]\cup s_1
     \quad
     \envnraenv \vdash q_2 \qapp d_1 \Downarrowa \true
     \quad
     \envnraenv \vdash \qselect{q_2}{s_1} \qapp d \Downarrowa s_2}
    \\[\jot]
    \infer[Sel_{\mbox{F}}]
      {\envnraenv \vdash \qselect{q_2}{q_1} \qapp d \Downarrowa s_2}
      {\envnraenv \vdash q_1 \qapp d \Downarrowa [d_1]\cup s_1
       \quad
       \envnraenv \vdash q_2 \qapp d_1 \Downarrowa \false
       \quad
       \envnraenv \vdash \qselect{q_2}{s_1} \qapp d \Downarrowa s_2}
    \qquad
    \infer[Sel_\emptyset]
      {\envnraenv \vdash q_1 \qapp d \Downarrowa \emptyset}
      {\envnraenv \vdash \qselect{q_2}{q_1} \qapp d \Downarrowa \emptyset}
    \\[\jot]
    \infer[Prod^{l}_{\emptyset}]
      {\envnraenv \vdash q_1\times q_2 \qapp d \Downarrowa \emptyset}
      {\envnraenv \vdash q_1 \qapp d \Downarrowa \emptyset}
    \qquad
    \infer[Prod^{r}_{\emptyset}]
      {\envnraenv \vdash q_1\times q_2 \qapp d \Downarrowa \emptyset}
      {\envnraenv \vdash q_2 \qapp d\Downarrowa \emptyset}
    \\[\jot]
    \infer[Prod]
      {\envnraenv \vdash q_1\times q_2 \qapp d \Downarrowa [d_1 \opconcat d_2]\cup s_3\cup s_4}
      {\envnraenv \vdash q_1 \!\qapp\! d\!\Downarrowa\! [d_1]\!\cup\! s_1
       \quad
       \envnraenv \vdash q_2 \!\qapp\! d\!\Downarrowa\! [d_2]\!\cup\! s_2
       \quad
       \envnraenv \vdash [d_1]\!\times\! s_2 \!\qapp\! d\!\Downarrowa\! s_3
       \quad
       \envnraenv \vdash s_1\!\times\! \left([d_2]\!\cup\! s_2\right) \!\qapp\! d\! \Downarrowa\! s_4}
    \\[\jot]
    \infer[Env]
      {\envnraenv \vdash \qENV \qapp\ d \Downarrowa \envnraenv}
      {}
    \qquad
    \infer[\mbox{Comp$^e$}]
      {\envnraenv_1 \vdash q_2 \circ^e q_1 \qapp\ d_1 \Downarrowa d_2}
      {\envnraenv_1 \vdash q_1 \qapp\ d_1 \Downarrowa \envnraenv_2
       \quad
       \envnraenv_2 \vdash q_2 \qapp\ d_1 \Downarrowa d_2}
    \\[\jot]
    \infer[\mbox{Map$^e_\emptyset$}]
      {\emptyset \vdash \qmapenv{q_2} \qapp d \Downarrowa \emptyset}
      {}
    \qquad
    \infer[\mbox{Map$^e$}]
      {[d_1]\cup s_1 \vdash \qmapenv{q_2} \qapp d \Downarrowa [d_2]\cup s_2}
      {d_1 \vdash q_2 \qapp d \Downarrowa d_2
       \quad
       s_1 \vdash \qmapenv{q_2} \qapp d \Downarrowa s_2}
    \\[\jot]
    \infer[\mbox{Default$_{\lnot\emptyset}$}]
      {\envnraenv \vdash q_1~\qor~q_2\qapp d \Downarrowa d_1}
      {\envnraenv \vdash q_1\qapp d \Downarrowa d_1
       \quad
       d_1 \neq \emptyset}
    \qquad
    \infer[\mbox{Default$_{\emptyset}$}]
      {\envnraenv \vdash q_1~\qor~q_2\qapp d \Downarrowa d_2}
      {\envnraenv \vdash q_1\qapp d \Downarrowa \emptyset
       \quad
       \envnraenv \vdash q_2\qapp d \Downarrowa d_2}
    \\[\jot]
    \infer[\mbox{Either$_{\dleft{}}$}]
      {\envnraenv \vdash \qeither{q_1}{q_2}\qapp {\dleft{}}\ d \Downarrowa d_1}
      {\envnraenv \vdash q_1\qapp d \Downarrowa d_1}
    \qquad
    \infer[\mbox{Either$_{\dright{}}$}]
      {\envnraenv \vdash \qeither{q_1}{q_2}\qapp {\dright{}}\ d \Downarrowa d_2}
      {\envnraenv \vdash q_2\qapp d \Downarrowa d_2}
  \end{gather*}
}
\end{minipage}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> fig/sqlalg-exp-semantics.tex <==

\begin{minipage}[c]{.4\linewidth}
{\footnotesize
\[
\def\arraystretch{1.2}
\begin{array}{lcl}
\seme{c}{\env} & = & $c$ \\
% \seme{a}{[]} & = & {\tt default} \hfill \hspace*{0.2cm}\mbox{if $a$ is an attribute} \\
% \seme{a}{(A, G, []) :: \env} & = & \seme{a}{\env}\\
\seme{a}{(A, G, T) :: \env} & = & T.a  \qquad\hspace*{0.5em}\mbox{if~} a \in A\\
\seme{a}{(A, G, T) :: \env} & = & \seme{a}{\env} \qquad\mbox{if~} a \notin A\\
\seme{\fn(\overline{e})}{\env} & = & \fn(\overline{\seme{e}{\env}}) \\
\seme{\ag(e)}{\env} & = & \ag\left(\overline{\seme{e}{((A,G,[t]) :: \env')}}\right)_{t\in T} \\
&&\mbox{if~} \findevalenv{\env}{e} = (A,G,T) :: \env'
\end{array}
\]
}
\end{minipage}
\qquad\quad
\begin{minipage}[c]{.4\linewidth}
{\footnotesize
\begin{tabular}[c]{@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}}
\infer{\findevalenv{\env}{c}  =  \env}{c \in \values} &
\multicolumn{2}{c}{\infer{\findevalenv{[]}{e}  =  {\tt undefined}}{e\notin\values}} \\[1.5ex]
\multicolumn{3}{c}{\infer{\findevalenv{((A,G,T) :: \env)}{e}  = \env'}{e\notin\values & \findevalenv{\env}{e} = \env' & \env' \neq {\tt undefined}}}\\[1.5ex]
\multicolumn{3}{c}{\infer{\findevalenv{((A,G,T) :: \env)}{e}  = (A,G,T) :: \env}{\findevalenv{\env}{e} = {\tt undefined} & {\isbuiltupon{(A \cup \bigcup_{(A',G,T)\in \env} G)}{e}}}}\\[1.5ex]
% \multicolumn{3}{c}{\infer{\isasuitableenv{A}{\env}{e}} {\isbuiltupon{(A \cup \bigcup_{(A',G,T)\in \env} G)}{e}}}\\[1.5ex]
\infer{\isbuiltupon{G}{c}}{c \in \values} &
\infer{\isbuiltupon{G}{e}}{e \in G} &
\infer{\isbuiltupon{G}{\fn(\overline e)}}{\bigwedge_{\overline{e}}\isbuiltupon{G}{e}}
\end{tabular}
}
\end{minipage}


% \begin{minipage}[c]{.4\linewidth}
% {\footnotesize
% \begin{tabular}[c]{@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}}
% \infer{\findevalenv{\env}{c}  =  \env}{c \in \values} &
% \multicolumn{2}{c}{\infer{\findevalenv{[]}{e}  =  {\tt undefined}}{e\notin\values}} \\[1.5ex]
% \multicolumn{3}{c}{\infer{\findevalenv{((A,G,T) :: \env)}{e}  = \env'}{e\notin\values & \findevalenv{\env}{e} = \env'}}\\[1.5ex]
% \multicolumn{3}{c}{\infer{\findevalenv{((A,G,T) :: \env)}{e}  = (A,G,T) :: \env}{\findevalenv{\env}{e} = {\tt undefined} & \isasuitableenv{A}{\env}{e}}}\\[1.5ex]
% \multicolumn{3}{c}{\infer{\isasuitableenv{A}{\env}{e}}{\isbuiltupon{(A \cup \bigcup_{(A',G,T)\in \env} G)}{e}}}\\[1.5ex]
% \infer{\isbuiltupon{G}{c}}{c \in \values} &
% \infer{\isbuiltupon{G}{e}}{e \in G} &
% \infer{\isbuiltupon{G}{\fn(\overline e)}}{\bigwedge_{\overline{e}}\isbuiltupon{G}{e}}
% \end{tabular}
% }
% \end{minipage}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> fig/sqlalg-formula-semantics.tex <==
{\footnotesize
\[
\setstretch{1.3}
\begin{array}[t]{l@{~}c@{~}l}
\semf{f_1 \mathtt{~and~} f_2}{\env}{i} & = & \semf{f_1}{\env}{i} \wedge_3 \semf{f_2}{\env}{i}\\
\semf{f_1 \mathtt{~or~} f_2}{\env}{i} & = & \semf{f_1}{\env}{i} \vee_3 \semf{f_2}{\env}{i}\\
\semf{\mathtt{not~} f}{\env}{i} & = & \neg{}_3 \semf{f}{\env}{i}\\
\semf{\mathtt{true}}{\env}{i} & = & \mathit{true}\\
\semf{p(\overline{e_n})}{\env}{i} & = & p(\overline{\sema{e_n}{\env}})\\
\end{array}
\quad
\begin{array}[t]{l@{~}c@{~}l}
\semf{p(\overline{e_n}, \mathtt{~all~} q)}{\env}{i} & = & \mathit{true}
~~{\mbox{iff~} \semf{p(\overline{e_n},t)}{\env}{i} = \mathit{true} \mbox{~for all~} t \in \semq{q}{\env}{i}}\\
\semf{p(\overline{e_n}, \mathtt{~any~} q)}{\env}{i} & = & \mathit{true}
~~{\mbox{iff~} \semf{p(\overline{e_n},t)}{\env}{i} = \mathit{true} \mbox{~and exists~} t \in \semq{q}{\env}{i}}\\
\semf{\overline{e_n \mathtt{~as~} a_n} \mathtt{~in~} q}{\env}{i} & = & \mathit{true}
~~{\mbox{if~} (\overline{a_n=\sema{e_n}{\env}}) \mbox{~belongs to~} \semq{q}{\env}{i}}\\
\semf{\mathtt{exists~} q}{\env}{i} & = & \mathit{true}
~~\mbox{iff~} \semq{q}{\env}{i} \mbox{~is not empty}
\end{array}
\]
}


%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:


==> fig/sqlalg-query-semantics.tex <==
{\footnotesize
\[
\setstretch{1.3}
\begin{array}[t]{l@{~}c@{~}l}
\semq{\mbox{\tt ()}}{\env}{i} & = & \{\!| ~ |\!\} \\
\semq{\mathit{tbl}}{\env}{i}  & = & i.\mathit{tbl} \quad \mbox{~if~} \mathit{tbl} \mbox{~is a table}\\
\semq{Q_1\mathtt{~union~} Q_2}{\env}{i} & = & \semq{Q_1}{\env}{i}\cup\semq{Q_2}{\env}{i}\\
\semq{Q_1\mathtt{~intersect~} Q_2}{\env}{i} & = & \semq{Q_1}{\env}{i}\cap\semq{Q_2}{\env}{i}\\
\semq{Q_1\mathtt{~except~} Q_2}{\env}{i} & = & \semq{Q_1}{\env}{i}\setminus\semq{Q_2}{\env}{i}\\
\semq{Q_1 ~{\Large \bowtie}~ Q_2}{\env}{i} & = & \\
\multicolumn{3}{l}{\left\{\!\left|\left(\overline{a_n=c_n},\overline{b_k=d_k}\right)
\left|
\begin{array}{l}
(\overline{a_n=c_n}) \in \semq{Q_1}{\env}{i} ~\wedge\\
(\overline{b_k=d_k}) \in \semq{Q_2}{\env}{i}  ~\wedge\\
(\forall~ n,k, ~~ a_n = b_k \Rightarrow c_n = d_k)
\end{array}
\right.\right|\!\right\}} \\
\end{array}
\hspace*{-0.9em}
\begin{array}[t]{l@{~}c@{~}l}
\semq{{\large \pi}_{(\overline{e_n \mathtt{\,as\,} a_n})}(Q)}{\env}{i} & = &
\{\!| (\overline{a_n = \seme{e_n}{(\ell(t),[],[t]) :: \env}}) \mid
t \in \semq{Q}{\env}{i}
|\!\}\\
%
\semq{{\large \sigma}_{f}(Q)}{\env}{i} & = &
\{\!|t\in\semq{Q}{\env}{i} \mid \semf{f}{(\ell(t),[],[t]) :: \env}{i} = \top|\!\}\\
%
\multicolumn{3}{l}{
\semq{{\large \gamma}_{(\overline{e_k \mathtt{\,as\,} a_k},\overline{e_n},f) }(Q)}{\env}{i} = } \\
\multicolumn{3}{c}{\left\{\!\left| \overline{(a_k=\seme{e_k}{(\ell(T),\overline{e_n},T)::\env})} | T\in\mathbb{F}_3 \right|\!\right\}} \\
\multicolumn{3}{@{\hspace{1cm}}l}{\mbox{and~} \mathbb{F}_2 \mbox{~is a partition of $\semq{Q}{\env}{i}$ according to $\overline{e_n}$} }\\
\multicolumn{3}{@{\hspace{1cm}}l}{\mbox{and~} \mathbb{F}_3 = \left\{\!\left|T \in {\mathbb F}_2  \left| \semf{f}{(\ell(T),\overline{e_n},T)::\env}{i} = \top\right.\right|\!\right\}} \\
\end{array}
\]
}

%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:


==> fig/sqlalg-semantics-summary.tex <==
{\footnotesize
\[
\setstretch{1.3}
\begin{array}[t]{l@{~}c@{~}l}
\semq{\mbox{\tt ()}}{\env}{i} & = & \{\!| ~ |\!\} \\
\semq{\mathit{tbl}}{\env}{i}  & = & i.\mathit{tbl} \quad \mbox{~if~} \mathit{tbl} \mbox{~is a table}\\
% \semq{Q_1\mathtt{~union~} Q_2}{\env}{i} & = & \semq{Q_1}{\env}{i}\cup\semq{Q_2}{\env}{i}\\
% \semq{Q_1\mathtt{~intersect~} Q_2}{\env}{i} & = & \semq{Q_1}{\env}{i}\cap\semq{Q_2}{\env}{i}\\
% \semq{Q_1\mathtt{~except~} Q_2}{\env}{i} & = & \semq{Q_1}{\env}{i}\setminus\semq{Q_2}{\env}{i}\\
  \semq{Q_1 ~{\Large \bowtie}~ Q_2}{\env}{i} & = & \\[\medskipamount]

\multicolumn{3}{l}{\left\{\!\left|\left(\overline{a_n=c_n},\overline{b_k=d_k}\right)
\left|
\begin{array}{l}
(\overline{a_n=c_n}) \in \semq{Q_1}{\env}{i} ~\wedge\\
(\overline{b_k=d_k}) \in \semq{Q_2}{\env}{i}  ~\wedge\\
(\forall~ n,k, ~~ a_n = b_k \Rightarrow c_n = d_k)
\end{array}
\right.\right|\!\right\}} \\
\end{array}
\hspace*{-5.9em}
\begin{array}[t]{l@{~}c@{~}l}
\semq{{\large \pi}_{(\overline{e_n \mathtt{\,as\,} a_n})}(Q)}{\env}{i} & = &
\{\!| (\overline{a_n = \seme{e_n}{(\ell(t),[],[t]) :: \env}}) \mid
t \in \semq{Q}{\env}{i}
|\!\}\\
%
\semq{{\large \sigma}_{f}(Q)}{\env}{i} & = &
\{\!|t\in\semq{Q}{\env}{i} \mid \semf{f}{(\ell(t),[],[t]) :: \env}{i} = \top|\!\}\\
%
\multicolumn{3}{l}{
\semq{{\large \gamma}_{(\overline{e_k \mathtt{\,as\,} a_k},\overline{e_n},f) }(Q)}{\env}{i} = } \\[\medskipamount]
\multicolumn{3}{@{\hspace{2cm}}l}{\left\{\!\left| \overline{(a_k=\seme{e_k}{(\ell(T),\overline{e_n},T)::\env})} | T\in\mathbb{F}_3 \right|\!\right\}} \\
\multicolumn{3}{@{\hspace{3cm}}l}{\mbox{and~} \mathbb{F}_2 \mbox{~is a partition of $\semq{Q}{\env}{i}$ according to $\overline{e_n}$} }\\
\multicolumn{3}{@{\hspace{3cm}}l}{\mbox{and~} \mathbb{F}_3 = \left\{\!\left|T \in {\mathbb F}_2  \left| \semf{f}{(\ell(T),\overline{e_n},T)::\env}{i} = \top\right.\right|\!\right\}} \\
\end{array}
\]
\smallskip
\[
\setstretch{1.3}
\begin{array}[t]{l@{~}c@{~}l}
  \semf{f_1 \mathtt{ ~and~} f_2}{\env}{i} & = & \semf{f_1}{\env}{i} \wedge_3 \semf{f_2}{\env}{i}\\
  \semf{f_1 \mathtt{ ~or~} f_2}{\env}{i} & = & \semf{f_1}{\env}{i} \vee_3 \semf{f_2}{\env}{i}\\
  % \semf{{\tt not~} f}{\env}{i} & = & \neg{}_3 \semf{f}{\env}{i}\\
  % \semf{{\tt true}}{\env}{i} & = & \mathit{true}\\
  \semf{p(\overline{e_n})}{\env}{i} & = & p(\overline{\sema{e_n}{\env}})\\
  \end{array}
  \quad
  \begin{array}[t]{l@{~}c@{~}l}
  \semf{p(\overline{e_n}, \mathtt{~all~} q)}{\env}{i} & = & \mathit{true}
  ~~{\mbox{iff~} \semf{p(\overline{e_n},t)}{\env}{i} = \mathit{true} \mbox{~for all~} t \in \semq{q}{\env}{i}}\\
  % \semf{p(\overline{e_n}, \mathtt{~any~} q)}{\env}{i} & = & \mathit{true}
  % ~~{\mbox{iff~} \semf{p(\overline{e_n},t)}{\env}{i} = \mathit{true} \mbox{~and exists~} t \in \semq{q}{\env}{i}}\\
  % \semf{\overline{e_n \mathtt{ ~as~} a_i} \mathtt{~in~} q}{\env}{i} & = & \mathit{true}
  % ~~{\mbox{if~} (\overline{a_i=\sema{e_n}{\env}}) \mbox{~belongs to~} \semq{q}{\env}{i}}\\
  \semf{\mathtt{exists~} q}{\env}{i} & = & \mathit{true}
  ~~\mbox{iff~} \semq{q}{\env}{i} \mbox{~is not empty}
  \end{array}
\]
\medskip
\[
\setstretch{1.3}
\begin{array}[t]{l@{~}c@{~}l}
  \seme{c}{\env} & = & $c$
\end{array}
\quad
\begin{array}[t]{l@{~}c@{~}l}
\seme{\fn(\overline{e})}{\env} & = & \fn(\overline{\seme{e}{\env}})
\end{array}
\quad
\begin{array}[t]{l@{~}c@{~}l}
  \seme{a}{(A, G, T) :: \env} & = &
  \left\lbrace
  \begin{array}[c]{@{~}ll}
   T.a  & \mbox{if~} a \in A\\
  \seme{a}{\env} & \mbox{if~} a \notin A
  \end{array}
  \right.
\end{array}
\]
% \quad
% \begin{minipage}[c]{.4\linewidth}
%   {\footnotesize
%   \[
%   \def\arraystretch{1.2}
%   \begin{array}{lcl}
%   \seme{c}{\env} & = & $c$ \\
%   % \seme{a}{[]} & = & \mathtt{default} \hfill \hspace*{0.2cm}\mbox{if $a$ is an attribute} \\
%   % \seme{a}{(A, G, []) :: \env} & = & \seme{a}{\env}\\
%   \seme{a}{(A, G, T) :: \env} & = & T.a  \qquad\hspace*{0.5em}\mbox{if~} a \in A\\
%   \seme{a}{(A, G, T) :: \env} & = & \seme{a}{\env} \qquad\mbox{if~} a \notin A\\
%   \seme{\fn(\overline{e})}{\env} & = & \fn(\overline{\seme{e}{\env}}) \\
%   \seme{\ag(e)}{\env} & = & \ag\left(\overline{\seme{e}{((A,G,[t]) :: \env')}}\right)_{t\in T} \\
%   &&\mbox{if~} \findevalenv{\env}{e} = (A,G,T) :: \env'
%   \end{array}
  % \]
  % }
  % \end{minipage}
  % \qquad\quad
  % \begin{minipage}[c]{.4\linewidth}
  % {\footnotesize
  % \begin{tabular}[c]{@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}}
  % \infer{\findevalenv{\env}{c}  =  \env}{c \in \values} &
  % \multicolumn{2}{c}{\infer{\findevalenv{[]}{e}  =  \mathtt{undefined}}{e\notin\values}} \\[1.5ex]
  % \multicolumn{3}{c}{\infer{\findevalenv{((A,G,T) :: \env)}{e}  = \env'}{e\notin\values & \findevalenv{\env}{e} = \env' & \env' \neq \mathtt{undefined}}}\\[1.5ex]
  % \multicolumn{3}{c}{\infer{\findevalenv{((A,G,T) :: \env)}{e}  = (A,G,T) :: \env}{\findevalenv{\env}{e} = \mathtt{undefined} & {\isbuiltupon{(A \cup \bigcup_{(A',G,T)\in \env} G)}{e}}}}\\[1.5ex]
  % % \multicolumn{3}{c}{\infer{\isasuitableenv{A}{\env}{e}} {\isbuiltupon{(A \cup \bigcup_{(A',G,T)\in \env} G)}{e}}}\\[1.5ex]
  % \infer{\isbuiltupon{G}{c}}{c \in \values} &
  % \infer{\isbuiltupon{G}{e}}{e \in G} &
  % \infer{\isbuiltupon{G}{\fn(\overline e)}}{\bigwedge_{\overline{e}}\isbuiltupon{G}{e}}
  % \end{tabular}
  % }
  % \end{minipage}
  

}

%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:


==> fig/sqlalg-syntax.tex <==
\[
\small
\begin{array}[t]{cc}
\begin{array}[t]{l@{\hspace*{0.5em}}c@{\hspace*{0.5em}}l}
\algquery & ::= & 
  \mbox{\tt ()} ~~|~~
  \mathit{tbl} \\ && |~~
  \algquery ~(\mathtt{union} ~~|~~ \mathtt{intersect} ~~|~~ \mathtt{except})~ \algquery ~~|~~
  \algquery ~{\large \bowtie}~ \algquery \\ && |~~
  {\large \pi}_{(\overline{e \mathtt{\,as\,} \attribute})}(\algquery) ~~|~~
  {\large \sigma}_{\formula}(\algquery) \\ && |~~
  {\large \gamma}_{(\overline{e \mathtt{\,as\,} \attribute}, \overline{e},\formula)}(\algquery) \\
\end{array}
&
\begin{array}[t]{l@{\hspace*{0.5em}}c@{\hspace*{0.5em}}l}
\formula & ::= &
  \mathtt{true} ~~|~~
  \formula ~(\mathtt{and} ~~|~~ \mathtt{or})~ \formula ~~|~~
  \mathtt{not}~ \formula \\ & & |~~
  p(\overline e) ~~|~~
  p(\overline e, (\mathtt{all} ~~|~~ \mathtt{any})~ {\algquery}) \\ & & |~~
  \overline{e ~\mathtt{as}~ \attribute}~ \mathtt{in}~ {\algquery} ~~|~~
  \mathtt{exists} ~{\algquery}
\\

e   & ::= & c ~~|~~ \attribute ~~|~~ \fn(\overline{e}) ~~|~~ \ag(\overline{e})
% \\
% \fn & ::= &
% \mathtt{+} ~|~ \mathtt{-} ~|~ \mathtt{*} ~|~ \mathtt{/} ~|~ ...
% \\
% \ag & ::= &
% \mathtt{sum} ~|~ \mathtt{avg} ~|~ \mathtt{min} ~|~ ...
% \\
\end{array}
\end{array}
\]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> fig/sqlatonrae-expressions-trans.tex <==

  % \begin{minipage}[c]{.8\linewidth}
    {\small
      \[
        \setstretch{1.3}
        \begin{array}{lcl}
          \trft{\aenv}{v} & = & \trval{v} \hfill \hspace*{0.6cm}
                                \mbox{if $v$ is a value}\\
          % \trft{[]}{a} & = & \trval{{\tt default}}
          %                    \hfill \hspace*{0.6cm}
          %                    \mbox{if $a$ is an attribute name}\\
          \trft{(A, G) :: \aenv}{a}
                          & = &
                                \tdot{{\tt first\_elt\_of}
                                (\tdot{\qENV}
                                {\mathit{slice}})}{\tratt{a}} \hfill
                                \hspace*{0.2cm}
                                \mbox{if~} a \in A \\
          \trft{(A, G) :: \aenv}{a}
                          & = & \trft{\aenv}{a}~\circ^{e}
                                ~(\tdot{\qENV}{\mathit{tail}})
                                \hfill \hspace*{0.2cm}
                                \mbox{if~} a \notin A \\
          \trft{\aenv}{\fn~(\overline{\ef})}
                          & = & \trfn{\fn}
                                {(\overline{\trft{\aenv}{\ef}})} \\
          \tra{\aenv}{\fn~(\overline{\ea})}
                          & = & \trfn{\fn}
                                {(\overline{\tra{\aenv}{\ea}})} \\
          \tra{\aenv}{\ag(\ef)}
                          & = &
                                \eapp{({\tt remove\_slices}
                                ~(\aenv,\ef))}
                                {\trag{\ag}
                                {(\overline{\trf{((A,G) :: \aenv')}
                                {\ef}})}}\\
          \multicolumn{3}{l}{\qquad\mbox{where~}
            {\tt remove\_slices}~(\aenv,\ef)
            ~~\mbox{removes the same number of slices as~}
            \findevalaenv{\aenv}{\ef}}
        \end{array}
      \]
    }
  % \end{minipage}

%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:


==> fig/sqlatonrae-formulae-trans.tex <==
  % \begin{minipage}[c]{.7\linewidth}
    {\small
      \[
        \setstretch{1.3}
        \begin{array}[t]{lcl}
          \trf{\aenv}{f_{1}~~\mathtt{and}~~f_{2}} & =
          & (\trf{\aenv}{f_{1}})~~\wedge_B~~(\trf{\aenv}{f_{2}})  \\
          \trf{\aenv}{f_{1}~~\mathtt{or}~~f_{2}} & =
          & (\trf{\aenv}{f_{1}})~~\vee_B~~(\trf{\aenv}{f_{2}}) \\
          \trf{\aenv}{ \mathtt{not}~~f} & =
          & \neg_B~~(\trf{\aenv}{f})  \\
          \trf{\aenv}{p~ (\overline{e})} & =
          &  \trp{p}{(\overline{\tre{\aenv}{e}})}  \\
          \trf{\aenv}{ \mathtt{true}} & =
          & \mathtt{true_B} \\
        \end{array}
        \quad
        \begin{array}[t]{lcl}
          \trf{\aenv}{p~~(e,\mathtt{all} ~~\algquery)} & =
          & \mathtt{all}_{B}~~p~~(\tre{\aenv}{e})~
            ~(\trq{\aenv}{\algquery})\\
          \trf{\aenv}{p~~(e,\mathtt{any} ~~\algquery)} & =
          & \mathtt{any}_B~~p~~(\tre{\aenv}{e})~
            ~(\trq{\aenv}{\algquery})\\
          \trf{\aenv}{ls~~ \mathtt{in}~~\algquery)} & =
          & (\trsel{\aenv}{ls})~~\mathtt{in}_B~
            ~(\trq{\aenv}{\algquery})\\
          \trf{\aenv}{\mathtt{exists} ~~\algquery} & =
          & \mathtt{count} ~
            ~(\trq{\aenv}{\algquery}) \mathtt{>} 0\\
        \end{array}
      \]
    }
  % \end{minipage}


%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:


==> fig/sqlatonrae-queries-trans-short.tex <==
%\begin{minipage}[c]{.9\linewidth}
    {\small
      \[
        \setstretch{1.3}
        \begin{array}{lcl}
          \trq{\aenv}{Q_1~~{\Large \bowtie}~~Q_2} & =
          & \trq{\aenv}{Q_1} \times \trq{\aenv}{Q_2}\\
          \trq{\aenv}{{\Large \sigma}_{f}(Q) } & =
          &  \qselect{\eapp{\pushd}{\trf{(\mathit{sort}~{Q},\{\})::\aenv}{f}}}
            {\trq{\aenv}{Q}}\\
          \trq{\aenv}{{\Large \pi}_{(\overline{e_n \mathtt{\,as\,} \attribute_n})} }(Q) & =
          & \qmap{\eapp{\pushd}
            {\trsel{(\mathit{sort}~{Q},\{\})::\aenv}{\overline{e_n \mathtt{\,as\,} \attribute_n}}}}
            {\trq{\aenv}{Q}} \\
           & & \\
          \trq{\aenv}{{\large \gamma}_{(\overline{e_n \mathtt{\,as\,} \attribute_n},\overline{b_k},f)}(Q) } & =
          & \text{let groups =}
            \qmap{\tdot{\qID}{g}}{\qgroupby{g}{\overline{b_k}}{\trq{\aenv}{Q}}}
            \text{in} \\
          & & \text{let filtered\_groups} = \qselect{\eapp{\pushq}
          {\trf{(\mathit{sort}~{Q},\overline{b_k})::\aenv}{f}}}
          {\text{groups}} \text{in} \\
          & &
          \qmap{\eapp{\pushq}
          {\trsel{(\mathit{sort}~{Q},\overline{b_k})::\aenv}{\overline{e_n \mathtt{\,as\,} \attribute_n}}}}
          {\text{filtered\_groups}}\\
          \multicolumn{3}{l}{\hspace*{9cm}\mbox{where}~g~
          \mbox{is a fresh label \wrt}~\overline{b_k}}\\
            %\hfill \hspace*{0.6cm}\mbox{if \dots}\\
        \end{array}
      \]
    }
%  \end{minipage}


%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:


==> fig/sqlatonrae-queries-trans.tex <==
  % \begin{minipage}[c]{.9\linewidth}
    {\small
      \[
        \setstretch{1.3}
        \begin{array}{lcl}
                    \trq{\aenv}{\mathit{tbl}} & =
          & \trtab{\mathit{tbl}}  \\
          \trq{\aenv}{Q_1~~\mathtt{union}~~Q_2} & =
          & \trq{\aenv}{Q_1}~~{ \cup}~~\trq{\aenv}{Q_2} \\
          \trq{\aenv}{Q_1~~\mathtt{intersect}~~Q_2} & =
          & \trq{\aenv}{Q_1}~~{ \cap}~~\trq{\aenv}{Q_2}\\
          \trq{\aenv}{Q_1~~\mathtt{except}~~Q_2} & =
          & \trq{\aenv}{Q_1}~~\mathtt{\setminus}~~\trq{\aenv}{Q_2} \\
          \trq{\aenv}{Q_1~~{\Large \bowtie}~~Q_2} & =
          & \trq{\aenv}{Q_1} \times \trq{\aenv}{Q_2}\\
          \trq{\aenv}{{\Large \sigma}_{f}(Q) } & =
          &  \qselect{\eapp{\pushd}{\trf{(\mathit{sort}~{Q},\{\})::\aenv}{f}}}
            {\trq{\aenv}{Q}}\\
          \trq{\aenv}{{\Large \pi}_{(\overline{e_n \mathtt{\,as\,} \attribute_n})} }(Q) & =
          & \qmap{\eapp{\pushd}
            {\trsel{(\mathit{sort}~{Q},\{\})::\aenv}{\overline{e_n \mathtt{\,as\,} \attribute_n}}}}
            {\trq{\aenv}{Q}} \\
          \trq{\aenv}{{\large \gamma}_{(\overline{e_n \mathtt{\,as\,} \attribute_n},\overline{b_k},f)}(Q) } & =
          & \\
          \multicolumn{3}{c}
          {\qquad\qmap{\eapp{\pushq}
          {\trsel{(\mathit{sort}~{Q},\overline{b_k})::\aenv}{\overline{e_n \mathtt{\,as\,} \attribute_n}}}}
          {\qselect{\eapp{\pushq}
          {\trf{(\mathit{sort}~{Q},\overline{b_k})::\aenv}{f}}}
          {\qmap{\tdot{\qID}{g}}{\qgroupby{g}{\overline{b_k}}{\trq{\aenv}{Q}}}}}}\\
          \multicolumn{3}{l}{\hspace*{1.6cm}\mbox{where}~g~
          \mbox{is a fresh label \wrt}~\overline{b_k}}
            %\hfill \hspace*{0.6cm}\mbox{if \dots}\\
        \end{array}
      \]
    }
  % \end{minipage}


%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-master: "../main"
%%% End:

